AutoSVA: Democratizing Formal Verification of RTL Module Interactions

Modern SoC design relies on the ability to separately verify IP blocks relative to their own specifications. Formal verification (FV) using SystemVerilog Assertions (SVA) is an effective method to exhaustively verify blocks at unit-level. Unfortunately, FV has a steep learning curve and requires engineering effort that discourages hardware designers from using it during RTL module development. We propose AutoSVA, a framework to automatically generate FV testbenches that verify liveness and safety of control logic involved in module interactions. We demonstrate AutoSVA's effectiveness and efficiency on deadlock-critical modules of widely-used open-source hardware projects.

==> txt/discussion.tex <==
\section{Discussion \label{sec:discussion}}

The implementation of \proj was done using Python and did not require any special Python libraries.
Each of the different parsing processes used regular expressions in order to flexibly accept different inputs for global parameter, signal, and annotation names and declarations.
Implementing this parsing process was the most challenging step because there are many different styles of writing RTL and the framework needed to strike a balance between complexity (to support more styles) and flexibility (to avoid too much specialization to a certain engineering style).
As a result, a fair number of rules were decided (see Section~\ref{sec:rules}) in order to avoid complexity while providing support for a wide range of parameters, signals, and annotations.

Implementing \proj{} and determining the usage rules was a multi-stage process that involved many iterations and reiterations of the design.
Testing \proj{} began with focusing on the smallest hardware module of DCP, the FIFO queue RTL design.
There were a few inconsistencies in the signal names that initially made parsing more difficult and revealed different scenarios (inputs) that the framework needed to account for.
For example, there were input signals that were not valid signals yet had a \texttt{val} suffix.
This threw off the ability to identify interfaces based on which signals corresponded to valid signals.
This also led to the suffixes rules (in Section~\ref{sec:rules}) in order to avoid confusion.

Additional implementation changes were necessary once \proj had successfully generated transactional models for the FIFO queue RTL and testing shifted to focus on the other hardware modules.
These changes were due to differences in how the other hardware modules were designed.
For example, the pipeline model introduced an additional property to ensure that there could only be one outstanding request at a time for certain fields.
The FIFO queue module did not require this property, so this was not supported at the time and needed to be added. 
These types of discoveries have led the current \proj implementation to be more modular and allow for further development to support properties beyond those in transactional models.
Such properties can include other liveness properties as well as safety properties.

Designing and developing \proj was a learning process. 
At the beginning of the project, many concepts in both SVA and formal verification with JasperGold were new, which made it more challenging to design a flexible framework.
However, as these concepts became more familiar, it became easier to consider different RTL designs and the liveness properties they would need verified.
